From Semantics to Types: the Case of the Imperative lambda-Calculus

We propose an intersection type system for an imperative lambda-calculus based on a state monad and equipped with algebraic operations to read and write to the store. The system is derived by solving a suitable domain equation in the category of omega-algebraic lattices; the solution consists of a filter-model generalizing the well-known construction for ordinary lambda-calculus. Then the type system is obtained out of the term interpretations into the filter-model itself. The so obtained type system satisfies the "type-semantics" property, and it is sound and complete by construction.

==> eptcsdata.tex <==
\providecommand{\firstpage}{168}
\providecommand{\publicationstatus}{Ana Sokolova (Eds.): MFPS 2021\\
EPTCS 351, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.351.11}{10.4204/EPTCS.351.11}}

